The A-shell star Phi Leo revisited: its photospheric and circumstellar spectra

Variable red- and blue-shifted absorption features observed in the Ca ii K line towards the A-type shell star $\phi$ Leo have been suggested by us in a previous work to be likely due to solid, comet-like bodies in the circumstellar (CS) environment. Our aim is to expand our observational study of this object to other characteristic spectral lines of A-type photospheres as well as to lines arising in their CS shells. We have obtained more than 500 high-resolution optical spectra collected at different telescopes from December 2015 to January 2019. We have analysed some photospheric lines, in particular Ca i 4226 \AA ~and Mg ii 4481 \AA, as well as the circumstellar shell lines Ca ii H\&K, Ca ii IR triplet, Fe ii, Ti ii, and the Balmer lines H$\alpha$ and H$\beta$. Our observational study reveals that $\phi$ Leo is a variable $\delta$ Scuti star whose spectra show remarkable dumps and bumps superimposed on the photospheric line profiles, which vary their strength and sharpness, propagate from blue- to more red-shifted radial velocities and persisting during a few hours, likely produced by non-radial pulsations. At the same time, all shell lines present an emission at $\sim$3 km/s centered at the core of the CS features, and two variable absorption minima at both sides of the emission. The variations observed in the Ca ii H\&K, Fe ii and Ti ii lines occur at any time scale from minutes to days and observing run, but without any clear correlation or recognizable temporal pattern among the different lines. In the case of H$\alpha$ the CS contribution is also variable in just one of the observing runs. We suggest that $\phi$ Leo is a rapidly rotating $\delta$ Scuti star surrounded by a variable, (nearly) edge-on CS disk possibly re-supplied by the $\delta$ Scuti pulsations.

==> Table_Observing_Log.tex <==
%% UNCOMMENT THE LINES BELOW IF YOU WANT TO RUN THE TABLE BY ITSELF
%%
%%
%%  \documentclass[structabstract]{aa}  
%%  %
%%  \usepackage{natbib}
%%  \usepackage{graphicx}
%%  \usepackage{lscape}
%%  \usepackage{longtable}
%%  \usepackage{txfonts}
%%  \usepackage{color}                           
%%  
%%  % This allows to number the tables as e.g. Table 3a, Table 3b, Table 3c ...
%%  \newcounter{subtable}
%%  %
%%  
%%  \begin{document}
%%
%% UNCOMMENT THE LINES ABOVE IF YOU WANT TO RUN THE TABLE BY ITSELF
%% AND ADD A LINE \end{document} AT THE VERY BOTTOM

\begin{center}

%% This command sends the beginning of the next table to the following page
\onecolumn

\begin{small}
\begin{longtable}{llllllll}
%\caption{Observing Log}
\multicolumn{8}{c}{{\bf \tablename\ \thetable{}.} Observing Log}
%This is the header for the first page of the table...  
\\
\hline
\hline
Date (UT)              & Instrument      & Date (UT)               & Instrument & Date (UT)               & Instrument & Date (UT)               & Instrument \\
\hline
\endfirsthead

%This is the header for the remaining page(s) of the table...
\multicolumn{2}{l}{{\bf \tablename\ \thetable{}}--continued} \\
\hline
\hline
 Date (UT)              & Instrument      & Date (UT)               & Instrument & Date (UT)               & Instrument & Date (UT)               & Instrument \\
\hline
\endhead

%This is the footer for all pages except the last page of the table...
\hline
\multicolumn{8}{l}{Continued\dots}\\
\endfoot

%This is the footer for the last page of the table...
\\
\endlastfoot
20151221T0627  & HERMES          &  20151223T0501  & HERMES      &  20151223T0614  & HERMES    &   20151223T0706  & HERMES      \\                    
20151223T0715  & HERMES          &  20151224T0524  & HERMES       &20160127T0411  & FIES             &  20160127T0536  & FIES  \\                     
20160128T0114  & HERMES          & 20160128T0126  & HERMES        &  20160129T0339  & HERMES    &  20160129T0510  & HERMES       \\                
20160129T0623  & HERMES          &  20160131T0220  & HERMES       &  20160131T0344  & HERMES    &  20160131T0451  & HERMES      \\                   
20160303T2343  & HERMES          &  20160303T2348  & HERMES       & 20160304T0300  & HERMES      &  20160304T0306  & HERMES      \\                   
20160304T2354  & HERMES          & 20160304T2359  & HERMES        &  20160305T0307  & HERMES     &  20160305T0314  & HERMES       \\                  
20160306T0016  & HERMES          &  20160306T0257  & HERMES       &  20160307T0010  & HERMES      &20160307T0213  & HERMES      \\                    
20160307T0224  & HERMES          &  20160326T0138  & FEROS          & 20160326T0312   & FEROS         &  20160326T0315  & FEROS      \\               
20160326T0553  & FEROS             & 20160327T0252  & FEROS            &  20160327T0449  & FEROS         &  20160327T0454  & FEROS       \\           
20160327T0601  & FEROS             &  20160328T0153  & FEROS           &  20160328T0346  & FEROS          &20160328T0548  & FEROS      \\             
20160329T0218  & FEROS             &  20160329T0340  & FEROS           &  20160329T0522  & FEROS          &  20160511T2021  & HERMES      \\          
20160511T2044  & HERMES          &20160511T2054  & HERMES          &  20160511T2105  & HERMES      &  20160511T2116  & HERMES       \\                
20160511T2127  & HERMES          &  20160511T2138  & HERMES        &  20160511T2151  & HERMES       &20160511T2202  & HERMES       \\                 
20160511T2213  & HERMES          &  20160511T2224  & HERMES        & 20160511T2234  & HERMES          &  20160511T2245  & HERMES       \\             
20160511T2317  & HERMES          & 20160511T2327  & HERMES          &  20160511T2338  & HERMES      &  20160511T2349  & HERMES        \\              
20160512T0000  & HERMES          &  20160512T0011  & HERMES        &  20160512T0020  & HERMES        &20170306T2245  & HERMES       \\                
20170306T2250  & HERMES          &  20170306T2301  & HERMES        & 20170306T2317  & HERMES          &  20170306T2333  & HERMES       \\             
20170306T2349  & HERMES          & 20170307T0005  & HERMES          &  20170307T0020  & HERMES      &  20170307T0036  & HERMES        \\              
20170307T0052  & HERMES          &  20170307T0108  & HERMES         &  20170307T0124  & HERMES        & 20170307T0140  & HERMES       \\              
20170307T0255  & HERMES          &  20170307T2215  & HERMES        & 620170307T2231  & HERMES          &  20170307T2247  & HERMES       \\              
20170307T2302  & HERMES          & 20170307T2323  & HERMES          &  20170307T2344  & HERMES      &  20170308T0005  & HERMES        \\              
20170308T0026  & HERMES          &  20170308T0047  & HERMES      &  20170308T0102  & HERMES        &20170308T0118  & HERMES       \\                  
20170308T0134  & HERMES          &  20170308T0150  & HERMES      & 20170308T0206  & HERMES          &  20170308T0222  & HERMES    \\                  
20170308T0237  & HERMES          & 20170308T0253  & HERMES          &  20170308T0309  & HERMES      &  20170308T0325  & HERMES   \\                   
20170308T0341  & HERMES          &  20170308T2219  & HERMES      &  20170308T2235  & HERMES      & 20170308T2251  & HERMES\\                          
20170308T2307  & HERMES      &  20170308T2323  & HERMES          & 20170308T2339  & HERMES          &  20170308T2354  & HERMES \\                     
20170309T0010  & HERMES      & 20170309T0026  & HERMES          &  20170309T0042  & HERMES      &  20170309T0058  & HERMES\\                          
20170309T0114  & HERMES          &  20170309T0129  & HERMES      &  20170309T0145  & HERMES       &20170309T0201  & HERMES\\                          
20170309T0303  & HERMES      &  20170309T0318  & HERMES       & 20170309T0334  & HERMES          &  20170309T0350  & HERME\\                          
20170309T0406  & HERMES      & 20170309T0422  & HERMES          &  20170309T0438  & HERMES      &  20170309T2210  & HERMES\\                          
20170309T2226  & HERMES          &  20170309T2242  & HERMES      &  20170309T2258  & HERMES      & 20170309T2314  & HERMES\\                          
20170309T2330  & HERMES      &  20170309T2345  & HERMES      & 20170310T0001  & HERMES          &  20170310T0017  & HERMES\\                          
20170310T0033  & HERMES      & 20170310T0049  & HERMES          &  20170310T0105  & HERMES      &  20170310T0120  & HERMES\\                          
20170310T0136  & HERMES          &  20170310T0152  & HERMES      &  20170310T0208  & HERMES      &20170310T0224  & HERMES \\                          
20170310T0240  & HERMES      &  20170310T0256  & HERMES      &20170310T0311  & HERMES          &  20170310T0327  & HERMES \\                          
20170310T0343  & HERMES      & 20170310T0359  & HERMES          &  20170310T0415  & HERMES      &  20170310T0431  & HERMES\\                          
20170310T0446  & HERMES          &  20170310T2202  & HERMES      &  20170310T2218  & HERMES      &20170310T2234  & HERMES \\                          
20170310T2249  & HERMES      &  20170310T2305  & HERMES      &20170310T2321  & HERMES          &  20170310T2337  & HERMES \\                          
20170310T2353  & HERMES      & 20170311T0009  & HERMES          &  20170311T0024  & HERMES      &  20170311T0040  & HERMES\\                          
20170311T0056  & HERMES          &  20170311T0112  & HERMES      &  20170311T0128  & HERMES      &20170311T0144  & HERMES \\                          
20170311T0159  & HERMES      &  20170311T0215  & HERMES      & 20170311T0231  & HERMES          &  20170311T0247  & HERMES\\                          
20170311T0303  & HERMES      & 20170311T0319  & HERMES          &  20170311T0334  & HERMES      &  20170311T0350  & HERMES\\                          
20170311T0406  & HERMES          &  20170311T0422  & HERMES      &  20170311T0438  & HERMES      &20170311T2219  & HERMES \\                          
20170311T2235  & HERMES      &  20170311T2251  & HERMES      & 20170311T2307  & HERMES          &  20170312T0131  & HERMES\\                          
20170312T0234  & HERMES      & 20170312T0250  & HERMES          &  20170312T0306  & HERMES      &  20170312T0322  & HERMES\\                          
20170312T0337  & HERMES          &  20170312T0353  & HERMES      &  20170312T0409  & HERMES      &20170312T0425  & HERMES \\                          
20170312T2215  & HERMES      &  20170312T2231  & HERMES      & 20170312T2247  & HERMES          &  20170312T2303  & HERMES\\                          
20170312T2318  & HERMES      & 20170312T2334  & HERMES          &  20170312T2350  & HERMES      &  20170313T0006  & HERMES\\                          
20170313T0022  & HERMES          &  20170313T0038  & HERMES      &  20170313T0053  & HERMES      &20170313T0109  & HERMES \\                          
20170313T0125  & HERMES      &  20170313T0141  & HERMES      & 20170313T0157  & HERMES          &  20170313T0213  & HERMES\\                          
20170313T0228  & HERMES      & 20170313T0244  & HERMES          &  20170313T0300  & HERMES      &  20170313T0316  & HERMES      \\                    
20170313T0332  & HERMES          &  20170313T0348  & HERMES      &  20170313T0403  & HERMES      & 20170313T0419  & HERMES  \\                        
20170313T2215  & HERMES      &  20170313T2231  & HERMES      & 20170313T2246  & HERMES          &  20170313T2302  & HERMES  \\                        
20170313T2318  & HERMES      & 20170313T2334  & HERMES          &  20170313T2350  & HERMES      &  20170314T0006  & HERMES  \\                        
20170314T0021  & HERMES          &  20170314T0037  & HERMES      &  20170314T0053  & HERMES      & 20170314T0109  & HERMES  \\                        
20170314T0125  & HERMES      &  20170314T0141  & HERMES      & 20170314T0156  & HERMES          &  20170314T0212  & HERMES  \\                        
20170314T0228  & HERMES      & 20170314T0244  & HERMES          &  20170314T0300  & HERMES      &  20170314T0316  & HERMES  \\                        
20170314T0331  & HERMES          &  20170314T0347  & HERMES      &  20170314T0403  & HERMES      & 20170314T0419  & HERMES  \\                        
20170328T2019  & HERMES      &  20170328T2035  & HERMES      & 20170328T2051  & HERMES          &  20170328T2107  & HERMES  \\                        
20170328T2123  & HERMES      & 20170328T2139  & HERMES          &  20170328T2154  & HERMES      &  20170328T2210  & HERMES  \\                        
20170328T2226  & HERMES          &  20170328T2242  & HERMES      &  20170328T2258  & HERMES      &20170328T2314  & HERMES   \\                        
20170328T2329  & HERMES      &  20170328T2345  & HERMES      &20170329T0001  & HERMES          &  20170329T0017  & HERMES   \\                        
20170329T0033  & HERMES      & 20170329T0049  & HERMES          &  20170329T0104  & HERMES      &  20170329T0120  & HERMES  \\                        
20170329T0136  & HERMES          &  20170329T0152  & HERMES      &  20170329T0208  & HERMES      & 20170329T0224  & HERMES  \\                        
20170329T2033  & HERMES      &  20170329T2049  & HERMES      & 20170329T2105  & HERMES          &  20170329T2121  & HERMES  \\                        
20170329T2137  & HERMES      & 20170329T2153  & HERMES          &  20170329T2208  & HERMES      &  20170329T2259  & HERMES  \\                        
20170329T2315  & HERMES          &  20170329T2330  & HERMES      &  20170329T2346  & HERMES      & 20170330T0002  & HERMES  \\                        
20170330T0018  & HERMES      &  20170330T0034  & HERMES      & 20170330T0050  & HERMES          &  20170330T0105  & HERMES  \\                        
20170330T0121  & HERMES      & 20170330T0137  & HERMES          &  20170330T0153  & HERMES      &  20170330T0209  & HERMES  \\                        
20170330T0225  & HERMES          &  20170330T0240  & HERMES      &  20170330T0256  & HERMES      &20170330T0312  & HERMES   \\                        
20170330T2035  & HERMES      &  20170330T2050  & HERMES      & 20170330T2106  & HERMES          &  20170330T2122  & HERMES  \\                        
20170330T2138  & HERMES      & 20170330T2154  & HERMES          &  20170330T2210  & HERMES      &  20170330T2225  & HERMES  \\                        
20170330T2241  & HERMES          &  20170330T2257  & HERMES      &  20170330T2313  & HERMES      & 20170330T2329  & HERMES  \\                        
20170330T2345  & HERMES      &  20170331T0001  & HERMES      & 20170331T0016  & HERMES          &  20170331T0032  & HERMES  \\                        
20170331T0048  & HERMES      & 20170331T0104  & HERMES          &  20170331T0120  & HERMES      &  20170331T0136  & HERMES  \\                        
20170331T0151  & HERMES          &  20170331T0207  & HERMES      &  20170331T0223  & HERMES      & 20170331T0239  & HERMES  \\                        
20170331T0255  & HERMES      &  20170331T0311  & HERMES      & 20170331T2103  & HERMES          &  20170331T2119  & HERMES  \\                        
20170331T2135  & HERMES      & 20170331T2151  & HERMES          &  20170331T2207  & HERMES      &  20170331T2252  & HERMES  \\                        
20170331T2258  & HERMES          &  20170331T2304  & HERMES      &  20170331T2310  & HERMES      & 20170331T2315  & HERMES  \\                        
20170331T2321  & HERMES      &  20170331T2327  & HERMES      & 20170331T2333  & HERMES          &  20170331T2339  & HERMES  \\                        
20170331T2345  & HERMES      & 20170331T2350  & HERMES          &  20170331T2356  & HERMES      &  20170401T0002  & HERMES  \\                        
20170401T0008  & HERMES          &  20170401T0014  & HERMES      &  20170401T0020  & HERMES      &20170401T0025  & HERMES      \\                     
20170401T0031  & HERMES      &  20170401T0037  & HERMES      & 20170401T0048  & HERMES          &  20170401T0104  & HERMES     \\                     
20170401T0120  & HERMES      & 20170401T0135  & HERMES          &  20170401T0151  & HERMES      &  20170401T0207  & HERMES     \\                     
20170401T0223  & HERMES          &  20170401T0239  & HERMES      &  20170401T0239  & FEROS        & 20170401T0255  & HERMES    \\                     
20170401T0304  & FEROS       &  20170401T0324  & FEROS           & 20170401T0350  & FEROS            &  20170401T0434  & FEROS \\                     
20170401T0513  & FEROS       & 20170401T0555  & FEROS           &  20170401T0629  & FEROS       &  20170401T2112  & HERMES     \\                     
20170401T2128  & HERMES          &  20170401T2144  & HERMES      &  20170401T2200  & HERMES      &20170401T2250  & HERMES      \\                     
20170401T2306  & HERMES      &  20170401T2322  & HERMES      & 20170401T2337  & HERMES          &  20170401T2353  & HERMES     \\                     
20170402T0009  & HERMES      & 20170402T0020  & FEROS           &  20170402T0025  & HERMES      &  20170402T0039  & FEROS      \\                     
20170402T0041  & HERMES          &  20170402T0055  & FEROS       &  20170402T0057  & HERMES      &20170402T0112  & HERMES      \\                     
20170402T0128  & HERMES      &  20170402T0144  & HERMES      & 20170402T0145  & FEROS           &  20170402T0200  & HERMES     \\                     
20170402T0203  & FEROS       & 20170402T0216  & HERMES          &  20170402T0218  & FEROS       &  20170402T0232  & HERMES     \\                     
20170402T0232  & FEROS           &  20170402T0248  & HERMES      &  20170402T0303  & HERMES      & 20170402T0325  & FEROS      \\                     
20170402T0330  & FEROS       &  20170402T0334  & FEROS       & 20170402T0400  & FEROS           &  20170402T0404  & FEROS      \\                     
20170402T0408  & FEROS       & 20170402T0423  & FEROS           &  20170402T0428  & FEROS       &  20170402T0432  & FEROS      \\                     
20170402T0500  & FEROS           &  20170402T0504  & FEROS       &  20170402T0508  & FEROS       & 20170402T0524  & FEROS      \\                     
20170402T0528  & FEROS       &  20170402T0532  & FEROS       & 20170402T0550  & FEROS           &  20170402T0554  & FEROS      \\                     
20170402T0558  & FEROS       & 20170402T0616  & FEROS           &  20170402T0620  & FEROS       &  20170402T0623  & FEROS      \\                     
20170402T2058  & HERMES          &  20170402T2114  & HERMES      &  20170402T2130  & HERMES      &20170402T2146  & HERMES      \\                     
20170402T2202  & HERMES      &  20170402T2252  & HERMES      & 20170402T2308  & HERMES          &  20170402T2323  & HERMES     \\                     
20170402T2339  & HERMES      & 20170402T2355  & HERMES          &  20170403T0011  & HERMES      &  20170403T0027  & HERMES     \\                     
20170403T0043  & HERMES          &  20170403T0051  & FEROS       &  20170403T0059  & HERMES      & 20170403T0107  & FEROS      \\                     
20170403T0114  & HERMES      &  20170403T0124  & FEROS       & 20170403T0130  & HERMES          &  20170403T0146  & HERMES     \\                     
20170403T0147  & FEROS       & 20170403T0202  & HERMES          &  20170403T0215  & FEROS       &  20170403T0218  & HERMES     \\                     
20170403T0229  & FEROS           &  20170403T0234  & HERMES      &  20170403T0246  & FEROS       & 20170403T0249  & HERMES     \\                     
20170403T0305  & HERMES      &  20170403T0336  & FEROS       & 20170403T0340  & FEROS           &  20170403T0344  & FEROS      \\                     
20170403T0359  & FEROS       & 20170403T0403  & FEROS           &  20170403T0407  & FEROS       &  20170403T0437  & FEROS      \\                     
20170403T0441  & FEROS           &  20170403T0445  & FEROS       &  20170403T0505  & FEROS       & 20170403T0509  & FEROS      \\                     
20170403T0513  & FEROS       &  20170403T0539  & FEROS       & 20170403T0543  & FEROS           &  20170403T0547  & FEROS      \\                     
20170403T0608  & FEROS       & 20170403T0622  & FEROS           &  20170403T0626  & FEROS       &  20170403T0630  & FEROS      \\                     
20170403T2048  & HERMES          &  20170403T2104  & HERMES      &  20170403T2119  & HERMES      & 20170403T2135  & HERMES     \\                     
20170403T2151  & HERMES      &  20170403T2241  & HERMES      & 20170403T2257  & HERMES          &  20170403T2313  & HERMES     \\                     
20170403T2329  & HERMES      & 20170403T2344  & HERMES          &  20170404T0000  & HERMES      &  20170404T0016  & HERMES     \\                     
20170404T0032  & HERMES          &  20170404T0048  & HERMES      &  20170404T0059  & FEROS       & 20170404T0104  & HERMES     \\                     
20170404T0119  & HERMES      &  20170404T0123  & FEROS       & 20170404T0135  & HERMES          &  20170404T0137  & FEROS      \\                     
20170404T0151  & HERMES      & 20170404T0155  & FEROS           &  20170404T0207  & HERMES      &  20170404T0223  & HERMES     \\                     
20170404T0234  & FEROS           &  20170404T0239  & HERMES      &  20170404T0253  & FEROS       & 20170404T0254  & HERMES     \\                     
20170404T0310  & HERMES      &  20170404T0337  & FEROS       & 20170404T0351  & FEROS           &  20170404T0430  & FEROS      \\                     
20170404T0507  & FEROS       & 20170404T0611  & FEROS           &  20170405T0035  & FEROS       &  20170405T0048  & FEROS      \\                     
20170405T0102  & FEROS           &  20170405T0120  & FEROS       &  20170405T0142  & FEROS       & 20170405T0209  & FEROS      \\                     
20170405T0224  & FEROS       &  20170405T0322  & FEROS        & 20170405T0353  & FEROS           &  20170405T0441  & FEROS     \\                     
20170405T0456  & FEROS       & 20170405T0520  & FEROS           &  20170405T0544  & FEROS       &  20170405T0557  & FEROS      \\                     
20170405T0613  & FEROS           &  20170405T0628  & FEROS       &  20170406T0027  & FEROS       & 20170406T0043  & FEROS      \\                     
20170406T0056  & FEROS       &  20170406T0115  & FEROS       & 20170406T0211  & FEROS           &  20170406T0231  & FEROS      \\                     
20170406T0257  & FEROS       & 20170406T0312  & FEROS           &  20170406T0325  & FEROS       &  20170406T0355  & FEROS      \\                     
20170406T0436  & FEROS           &  20170406T0457  & FEROS       &  20170406T0556  & FEROS       & 20170406T0612  & FEROS      \\                     
20170406T0645  & FEROS       &  20170406T0647  & FEROS       & 20170407T0148  & FEROS           &  20170407T0202  & FEROS      \\                     
20170407T0218  & FEROS       & 20170407T0232  & FEROS           &  20170407T0256  & FEROS       &  20170407T0323  & FEROS      \\                     
20170407T0338  & FEROS           &  20170407T0355  & FEROS       &  20170407T0409  & FEROS       & 20170407T0448  & FEROS      \\                     
20170407T0520  & FEROS       &  20170407T0538  & FEROS       & 20170407T0621  & FEROS           &  20170408T0054  & FEROS      \\                     
20170408T0107  & FEROS       & 20170408T0121  & FEROS           &  20170408T0133  & FEROS       &  20170408T0152  & FEROS      \\                     
20170408T0218  & FEROS           &  20170408T0231  & FEROS       &  20170408T0245  & FEROS       & 20170408T0316  & FEROS      \\                     
20170408T0347  & FEROS       &  20170408T0408  & FEROS       & 20170408T0507  & FEROS           &  20170408T0537  & FEROS      \\                     
20170408T0555  & FEROS       & 20170408T0610  & FEROS           &  20170408T0630  & FEROS       &  20170409T0056  & FEROS      \\                     
20170409T0113  & FEROS           &  20170409T0213  & FEROS       &  20170409T0232  & FEROS       & 20170409T0246  & FEROS      \\                     
20170409T0307  & FEROS       &  20170409T0333  & FEROS       & 20170409T0347  & FEROS           &  20170409T0403  & FEROS      \\                     
20170409T0428  & FEROS       & 20170409T0447  & FEROS           &  20170409T0544  & FEROS       &  20170409T0605  & FEROS      \\                     
20170409T0620  & FEROS           &  20170409T0636  & FEROS       &  20190130T0101  & HARPS-N    &20190130T0116  & HARPS-N      \\                     
20190130T0132  & HARPS-N     &  20190130T0147  & HARPS-N     & 20190130T0203  & HARPS-N         &  20190130T0218  & HARPS-N    \\                     
20190130T0234  & HARPS-N     & 20190130T0249  & HARPS-N         &  20190130T0305  & HARPS-N     &  20190130T0320  & HARPS-N    \\                     
20190130T0336  & HARPS-N         &  20190130T0351  & HARPS-N     &  20190130T0407  & HARPS-N     &20190130T0425  & HARPS-N     \\
\hline
\noalign{\smallskip}
\multicolumn{8}{l}{yyyymmddThhmm: yyyy, mm and dd are year, month and day; hh mm are the UT hour and minute of the beginning of the observation.}\\ 
\multicolumn{8}{l}{The items in the table are ordered from left to right and top to bottom.}
\label{obslog}
\end{longtable}
\end{small}
\end{center}


